Differentially Private Matrix Completion Revisited

We provide the first provably joint differentially private algorithm with formal utility guarantees for the problem of user-level privacy-preserving collaborative filtering. Our algorithm is based on the Frank-Wolfe method, and it consistently estimates the underlying preference matrix as long as the number of users $m$ is $\omega(n^{5/4})$, where $n$ is the number of items, and each user provides her preference for at least $\sqrt{n}$ randomly selected items. Along the way, we provide an optimal differentially private algorithm for singular vector computation, based on the celebrated Oja's method, that provides significant savings in terms of space and time while operating on sparse matrices. We also empirically evaluate our algorithm on a suite of datasets, and show that it consistently outperforms the state-of-the-art private algorithms.

==> contribution.tex <==
% !TEX root =PrivateMatrixCompletion.tex
\subsection{Our contributions}
\label{sec:contrib}

In this section, we provide a brief description of our main contributions in this work.

\mypar{Formalizing the joint model of computation} One of the main contributions of this work is to formalize the joint model of computation, and demonstrate the efficacy of this model. The joint model was introduced in \cite{MM09}, but has never been formally studied in the context of matrix completion. We show that  one can obtain strong error guarantees (i.e., empirical risk in Frobenius norm, and generalization error) for matrix completion  in this model under row differential privacy. Under row privacy, the complete row of the revealed matrix $\pomega(Y^*)$ is considered to be private information. The joint model helps to bypass some of the strong lower bounds from \cite{HR12}, and provides non-trivial error guarantees under row privacy.

In the joint model of computation, each row of the revealed matrix $\pomega(Y^*)$ belongs to an individual (client), and can be potentially sensitive. The objective is to learn a differentially private matrix $W^{\sf priv}$ from all the rows of the matrix $\pomega(Y^*)$, which can then be used by each client $i$ to complete her row $Y^{\sf priv}_i$ corresponding  to $\pomega(Y^*)_i$. Notice that client $i$ never directly reveals her completed row  $Y^{\sf priv}_i$ globally. The information flow is depicted in Figure \ref{fig:JointModel}.

\begin{figure*}[ht]
	\vskip 0.2in
	\begin{center}
		\centerline{\includegraphics[scale=0.3]{JointModel}}
		\caption{Joint model of computation: Using the information sent by each client (i.e., $\{{\sf row}_1,\cdots,{\sf row}_m\}$), the server computes $W_{\sf priv}$ under differential privacy. Then, each client $i$ creates her individual output $Y^i_{\sf priv}$ using $W_{\sf priv}$. Client $i$ never shares $Y^i_{\sf priv}$ directly with the server. The solid arrows pointing towards the server correspond to the information shared by each client $i$ with the server, and the dotted lines correspond to the differentially private information released by the server globally.}
		\label{fig:JointModel}
	\end{center}
	\vskip -0.2in
\end{figure*}

\mypar{Private matrix completion via Frank-Wolfe (Section \ref{sec:localLearning})} We use the classic Frank-Wolfe algorithm \cite{FW56}  from the optimization literature to solve the problem of differentially private matrix completion. The main analysis is in line with some of the recent works on matrix completion in the non-private setting \cite{tewari2011greedy,shalev2011large,jaggi2010simple}. Consider the hidden matrix $Y^*$ (with each entry in $[-1,1]$), and let $\Omega$ be a set of revealed entries from $Y^*$. Recall that $\pomega(\cdot)$ is an operator on a matrix which assigns zero to all the entries in the matrix which are not in the set $\Omega$.  Let \emph{$k$ be the nuclear norm (sum of the singular values)} bound on $Y^*$. The objective is to generate a matrix $Y^{\sf priv}$ with nuclear norm at most $k$ and rank at most $r$ (under differential privacy in the joint model) such that the empirical risk, which is $\pomega(Y^{\sf priv}-Y^*)$ in the squared Frobenius norm, is minimized. \cite{shalev2011large} show that using the squared Frobenius norm for bounding $\pomega(Y^{\sf priv}-Y^*)$ is sufficient to achieve generalization error guarantees. In the following, we state the an informal error guarantee (hiding the privacy parameters and logarithmic terms).

\begin{theorem}[Informal version of Theorem \ref{thm:utilRransferLearning}] Assume $|\Omega|=m\sqrt n$, and $\Omega$ is sampled uniformly at random. Then, there exists matrix $Y^{\sf priv}$ (with nuclear norm at most $k$ and rank at most $r$) in the joint model of computation under differential privacy, such that $$\frac{1}{2|\Omega|}\lfrob{\pomega(Y^{\sf priv}-Y^*)}^2=\frac{1}{m\sqrt n}\widetilde O\left(\frac{k^2}{r}+k\sqrt{nr^{1/2}}\right).$$
\end{theorem}

Let us define generalization error as $\E_{ij}\left[(Y^{\sf priv}_{ij}-Y^*_{ij})^2\right]$, where $i\in[m]$ and $j\in[n]$ are picked uniformly at random. If we set $k=\sqrt{mn}$, $r= \sqrt{n}$ and assume $m=\omega\left(n^{5/4}\right)$, then one can show that the generalization error is $o(1)$.  The above setting of parameters is fairly standard in the matrix completion literature \cite{shalev2011large}.

\mypar{Private matrix completion via Singular Value Decomposition (SVD) (Section \ref{sec:SVDapprox})} In this work, we consider a natural algorithm similar to an SVD-based private matrix completion algorithm proposed by \cite{MM09}. The algorithm in \cite{MM09}  first obtains a differentially private approximation to the right-singular subspace of $\pomega(Y^*)$, and then each client computes her corresponding row of $Y^{\sf priv}$ using a nearest neighbor search. Their results were empirical in nature without formal utility guarantees. In this work, we analyze a similar algorithm, except that the rows of $Y^{\sf priv}$ are computed by projecting individual rows of $\pomega(Y^*)$ to the right-singular subspace of $Y^{\sf priv}$ (which can easily be computed under differential privacy). We obtain the following utility guarantee:

\begin{theorem}[Informal version of Theorem \ref{thm:privSVD}] Assume $|\Omega|=m\sqrt n$, and $\Omega$ is sampled uniformly at random.  Then there exist an $Y^{\sf priv}$ of rank at most $r$ in the joint model of computation under differential privacy, such that
	\begin{align*}
	\frac{1}{2|\Omega|}\lfrob{\pomega(Y_{\sf priv}-Y^*)}^2\leq \frac{1}{2|\Omega|}\lfrob{\pomega(Y^*)-\pomega(Y^*)_r}^2+O\left(\frac{r\sqrt{n}}{m}\min\left\{1,\frac{n}{\sigma_r^2-\sigma_{r+1}^2}\right\}\right).
	\end{align*}
	Here,  $\sigma_r$ and $\sigma_{r+1}$ are the $r$-th and $(r+1)$-th singular values of $\pomega(Y^*)$, and $\pomega(Y^*)_r$ is the best rank-$r$ approximation to $\pomega(Y^*)$.
\end{theorem}
Notice that bound above depends on rank-$r$ approximation of the sampled matrix $\pomega(Y^*)$ in the worst-case, which may be bad even if $Y^*$ has good rank-$r$ approximation. However, if we assume incoherence in the matrix $Y^*$ (i.e., the right and the left singular subspaces have low-correlation with any of the standard basis vectors), then the low-rank empirical risk of $\pomega(Y^*)$ can be bounded in terms of the low-rank empirical risk of  $Y^*$. In terms of generalization error, if we consider $m=\omega(n)$, $\ltwo{Y^*}=\sqrt{m}$,  and the incoherence parameter $\mu=O(1)$, then  the generalization error bound translates to $o\left(1\right)$. Here, we set the rank parameter $r=\sqrt{n}$, which is the same rank of $Y^{\sf priv}$ in the Frank-Wolfe based case above.  To compare, although the sample complexity of $m$ for $o(1)$ generalization error is better for the SVD-based algorithm than the Frank-Wolfe based algorithm, this bound depends on an additional data-dependent property of incoherence $\mu$. 

\mypar{Extension to local differential privacy (Section \ref{sec:localmodel})} Local differential privacy \cite{EGS03,DJW13,BS15} is a stricter version of differential privacy, where the server is not trusted. Any communication from a client to the server is ensured to be differentially private w.r.t. the client's data record. In other words, each solid arrow in Figure \ref{fig:JointModel} would refer to a differentially private computation w.r.t. to each data record ( ${\sf row}_i$). Local differential privacy has received significant attention from companies like Google and Apple in the recent past \cite{erlingsson2014rappor,apple}. Both of our algorithms immediately extend to the local model, albeit an additional factor of $\sqrt{m}$ in the scale of the noise gets added for differential privacy%, where $m$ is the number of data records (rows of the matrix $Y^*$)
.

In the local model, there is a significant engineering advantage of using the SVD based algorithm, as compared to the Frank-Wolfe based algorithm. The former is completely non-interactive (i.e., it does not need to interact with the clients more than once), while the latter requires many rounds of interaction with the clients. In practical deployment, rounds of interaction can become a computational bottleneck. As a result, it may be advantageous to execute the SVD-based algorithm, even though its error bounds are weaker in the worst case.
